Bug Hunting By Computing Range Reduction

We describe a method of model checking called Computing Range Reduction (CRR). The CRR method is based on derivation of clauses that reduce the set of traces of reachable states in such a way that at least one counterexample remains (if any). These clauses are derived by a technique called Partial Quantifier Elimination (PQE). Given a number n, the CRR method finds a counterexample of length less or equal to n or proves that such a counterexample does not exist. We show experimentally that a PQE-solver we developed earlier can be efficiently applied to derivation of constraining clauses for transition relations of realistic benchmarks. One of the most appealing features of the CRR method is that it can potentially find long counterexamples. This is the area where it can beat model checkers computing reachable states (or their approximations as in IC3) or SAT-based methods of bounded model checking. PQE cannot be efficiently simulated by a SAT-solver. This is important because the current research in model checking is dominated by SAT-based algorithms. The CRR method is a reminder that one should not put all eggs in one basket.

==> induct_cond.fig.tex <==
%
% InductCond
%
\setlength{\intextsep}{2pt}
\setlength{\textfloatsep}{10pt}
%\begin{wrapfigure}{L}{2.1in}
\begin{figure}
%\begin{center}
\small
%\normalsize
%\vspace{-10pt}
\begin{tabbing}
aaa\=bb\=cc\= dd\= \kill
$\mi{InductCond}(\rr,\ur,\mi{k})$\{\\
\tb{\scriptsize{1}}\>  $j := k-1$;\\
\tb{\scriptsize{2}}\>  while ($\mi{true}$) \{\\
\tb{\scriptsize{3}}\Tt   if ($j = 1$) return($\mi{false}$); \\
\tb{\scriptsize{4}}\Tt   if $(\Impl{(\overline{H}_k \wedge U_k)}{(\overline{H}_j \wedge U_j)})$ \\
\tb{\scriptsize{5}}\ttt    return($\mi{true}$);\\
\tb{\scriptsize{6}}\Tt  $j := j-1$;\}\} \\
\end{tabbing} 
%\vspace{-20pt}
\caption{The \ti{InductCond} procedure}
\label{fig:induct_cond}
\end{figure}
%\end{wrapfigure}




==> junk.tex <==
\vspace{50pt}
dfdfdfdf
\clearpage
dffdfdfd
\clearpage

